A Fused Gromov-Wasserstein Framework for Unsupervised Knowledge Graph Entity Alignment

Entity alignment is the task of identifying corresponding entities across different knowledge graphs (KGs). Although recent embedding-based entity alignment methods have shown significant advancements, they still struggle to fully utilize KG structural information. In this paper, we introduce FGWEA, an unsupervised entity alignment framework that leverages the Fused Gromov-Wasserstein (FGW) distance, allowing for a comprehensive comparison of entity semantics and KG structures within a joint optimization framework. To address the computational challenges associated with optimizing FGW, we devise a three-stage progressive optimization algorithm. It starts with a basic semantic embedding matching, proceeds to approximate cross-KG structural and relational similarity matching based on iterative updates of high-confidence entity links, and ultimately culminates in a global structural comparison between KGs. We perform extensive experiments on four entity alignment datasets covering 14 distinct KGs across five languages. Without any supervision or hyper-parameter tuning, FGWEA surpasses 21 competitive baselines, including cutting-edge supervised entity alignment methods. Our code is available at https://github.com/squareRoot3/FusedGW-Entity-Alignment.

==> ACL23 Entity Alignment Camera Ready/tab_data.tex <==

\begin{table}[t!]
% \resizebox{\linewidth}{!}{
\small
\centering
\begin{tabular}{ccccc}  \toprule
Name                        & Lang.     & $|\mc E|$  & $|\mc R|$ & $|\mc T_r|$  \\\midrule
\multirow{2}{*}{DBP15K$_\textnormal{ZH\_EN}$} & ZH & 19,388 & 1,701 & 70,414  \\
                                 & EN & 19,572 & 1,323 & 95,142  \\
\multirow{2}{*}{DBP15K$_\textnormal{JA\_EN}$} & JA & 19,814 & 1,299 & 77,214  \\
                                 & EN & 19,780 & 1,153 & 93,484  \\
\multirow{2}{*}{DBP15K$_\textnormal{FR\_EN}$} & FR & 19,661 & 903   & 105,998 \\
                                 & EN & 19,993 & 1,208 & 115,722 \\\midrule
\multirow{2}{*}{SRPRS$_\textnormal{EN\_FR}$}  & EN & 15,000 & 177   & 33,532  \\
                                 & FR & 15,000 & 221   & 36,508  \\
\multirow{2}{*}{SRPRS$_\textnormal{EN\_DE}$}  & EN & 15,000 & 120   & 37,377  \\
                                 & DE & 15,000 & 222   & 38,363  \\\midrule
\multirow{2}{*}{D-W-15K-V2}      & EN & 15,000 & 167   & 73,983  \\
                                 & EN & 15,000 & 121   & 83,365  \\\midrule
\multirow{2}{*}{Med-BBK-9K}      & ZH & 9,162  & 32    & 158,357 \\
                                 & ZH & 9,162  & 20    & 50,307  \\\bottomrule
\end{tabular}
% }
% \vspace{-2mm}
\caption{Dataset statistics. $|\mc E|$, $|\mc R|$ and $|\mc T_r|$ represent the number of entities, relation types and relation triplets in each KG, respectively.}\label{tab:data}
% \vspace{-5mm}
\end{table}

==> ACL23 Entity Alignment Camera Ready/tab_exp1.tex <==
\begin{table*}[t!]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccl|ccc|ccc|ccc}\toprule
    &   \multicolumn{4}{|c}{Configurations}     & \multicolumn{3}{|c|}{DBP15K$_\textnormal{ZH\_EN}$}                  & \multicolumn{3}{c|}{DBP15K$_\textnormal{JA\_EN}$}                  & \multicolumn{3}{c}{DBP15K$_\textnormal{FR\_EN}$} \\
Model      & Name & Attr. & Trans. & Sup. & Hit1           & Hit10          & MRR            & Hit1           & Hit10          & MRR            & Hit1           & Hit10          & MRR            \\\midrule
JAPE       & \xmark   & \checkmark   & \xmark    & 30\%   & 0.412          & 0.745          & 0.490          & 0.363          & 0.685          & 0.476          & 0.324          & 0.667          & 0.430          \\
GCNAlign  & \xmark  & \cmark  & \xmark    & 30\%   & 0.413          & 0.744          & 0.549          & 0.399          & 0.745          & 0.546          & 0.373          & 0.745          & 0.532          \\
\textbf{FGWEA}       & \xmark  & \cmark  & \xmark    & 0\%    & \textbf{0.929} & \textbf{0.978} & \textbf{0.948} & \textbf{0.922} & \textbf{0.974} & \textbf{0.942} & \textbf{0.967} & \textbf{0.994} & \textbf{0.978} \\\midrule
GMatch & \cmark & \xmark   & \xmark    & 30\% & 0.679          & 0.785          & -              & 0.740          & 0.872          & -              & 0.894          & 0.952          & -              \\
SelfKG     & \cmark & \xmark   & \xmark    & 0\%    & 0.745          & 0.866          & -              & 0.816          & 0.913          & -              & 0.957          & 0.992          & -              \\
\textbf{FGWEA}       & \cmark & \xmark   & \xmark    & 0\%    & \textbf{0.926}          & \textbf{0.967}          & \textbf{0.942}          & \textbf{0.954}          & \textbf{0.981}          & \textbf{0.964}          & \textbf{0.996}          & \textbf{0.999}          & \textbf{0.997}          \\\midrule
RDGCN      & \cmark & \xmark   & \cmark   & 30\% & 0.708          & 0.846          & 0.746          & 0.767          & 0.895          & 0.812          & 0.886          & 0.957          & 0.911          \\
DATTI      & \cmark & \xmark   & \cmark   & 0\%    & 0.890          & 0.958          & -              & 0.921          & 0.971          & -              & 0.979          & 0.990          & -              \\
SEU        & \cmark & \xmark   & \cmark   & 0\%    & 0.900          & 0.965          & 0.924          & 0.956          & 0.991          & 0.969          & 0.988          & 0.999          & 0.992          \\
EASY       & \cmark & \xmark   & \cmark   & 0\%    & 0.898          & 0.979          & 0.930           & 0.943          & 0.990          & 0.960           & 0.980          & 0.998          & 0.990           \\
CPL-OT     & \cmark & \xmark   & \cmark   & 0\%    & 0.927          & 0.964          & 0.940           & 0.956          & 0.983          & 0.970           & 0.990          & 0.994          & 0.990           \\
UED      & \cmark & \xmark   & \cmark   & 0\%    & 0.915          & -          &-           & 0.941          & -          & -           & 0.984          & -         & -           \\
LightEA    & \cmark & \xmark   & \cmark   & 0\%    & 0.952          & \textbf{0.984} & 0.964          & 0.981          & \textbf{0.997} & \textbf{0.987} & \textbf{0.995} & 0.998          & \textbf{0.996} \\
\textbf{FGWEA}       & \cmark & \xmark   & \cmark   & 0\%    & \textbf{0.959} & 0.983 & \textbf{0.969} & \textbf{0.982} & 0.995          & \textbf{0.987} & 0.994 & \textbf{0.999} & \textbf{0.996} \\\midrule
AttrGNN    & \cmark & \cmark  & \xmark    & 30\% & 0.796          & 0.929          & 0.845          & 0.783          & 0.921          & 0.834 & 0.919          & 0.978          & 0.910          \\
BERT-INT*  & \cmark & \cmark  & \xmark    & 30\% & 0.968          & 0.990          & 0.977          & 0.964          & 0.991          & 0.975      & 0.992          & 0.998          & 0.995          \\
ICLEA      & \cmark & \cmark  & \xmark    & 0\%    & 0.884          & 0.972          & -              & 0.924          & 0.978          & -              & 0.991          & 0.999          & -              \\
\textbf{FGWEA}       & \cmark & \cmark  & \xmark    & 0\%    & \textbf{0.976} & \textbf{0.994} & \textbf{0.983} & \textbf{0.978} & \textbf{0.992} & \textbf{0.988} & \textbf{0.997} & \textbf{0.999} & \textbf{0.998} \\\midrule
MCLEA*    & \cmark & \cmark  & \cmark   & 30\% & 0.972          & 0.996          & 0.981          & 0.986          & \textbf{0.999} & 0.991          & 0.997          & \textbf{1.000} & 0.998          \\
\textbf{FGWEA}       & \cmark & \cmark  & \cmark   & 0\%    & \textbf{0.987} & \textbf{0.997} & \textbf{0.991} & \textbf{0.991} & 0.998          & \textbf{0.994} & \textbf{0.998} & \textbf{1.000}          & \textbf{0.999} \\\bottomrule
\end{tabular}
}
\caption{Evaluation Results of all compared EA methods on DBP15K under different configurations. Name, Attr., and Trans. represent the usage of entity name, attributes, and translation information, respectively. Sup. indicates the ratio of entity links for supervision. Methods marked with * use additional information not in DBP15K.}
% \vspace{-5mm}
\label{tab:exp1}
\end{table*}

==> ACL23 Entity Alignment Camera Ready/tab_exp2.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|cc|cc}\toprule
              & \multicolumn{2}{c|}{SRPRS$_\textnormal{EN\_FR}$}                     & \multicolumn{2}{c}{SRPRS$_\textnormal{EN\_DE}$}                     \\
Model        & Hit1            & Hit10          & Hit1            & Hit10          \\\midrule
% RDGCN*        & 0.672           & 0.767          & 0.779           & 0.886          \\
BERT-INT      & 0.971           & 0.975          & 0.986           & 0.988          \\\midrule
CPL-OT        & 0.974           & 0.988          & 0.974           & 0.989          \\
EASY*         & 0.965           & 0.989          & 0.974           & 0.992          \\
SEU*          & 0.982           & 0.995          & 0.983           & 0.996          \\
LightEA*      & 0.986           & 0.994          & 0.988           & 0.995          \\\midrule
\textbf{FGWEA} & \textbf{0.996}  & \textbf{0.999} & \textbf{0.997}  & \textbf{1.000} \\\bottomrule
\end{tabular}
}
% \vspace{-2mm}
\caption{Evaluation Results on the SPARS dataset. Methods marked with * used the translated entity name.}\label{tab:exp2}
% \vspace{-2mm}
\end{table}


==> ACL23 Entity Alignment Camera Ready/tab_exp3.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}\toprule
        & \multicolumn{3}{c|}{D-W-15K-V2}                & \multicolumn{3}{c}{MED-BBK-9K}                     \\
Model   & P             & R             & $F_1$            & P             & R             & $F_1$            \\\midrule
MultiKE & 49.5          & 49.5          & 49.5          & 41.0          & 41.0          & 41.0          \\
BootEA  & 82.1          & 82.1          & 82.1          & 30.7          & 30.7          & 30.7          \\
RSNs    & 72.3          & 72.3          & 72.3          & 19.5          & 19.5          & 19.5          \\\midrule
StrMatch  & 60.6          & 41.9          & 49.5          & 54.5          & 49.5          & 51.9          \\
LogMap  & -             & -             & -             & 86.4          & 44.1          & 58.4          \\
PARIS   & 95.0          & 85.0          & 89.7          & 77.9          & 36.7          & 49.9          \\
PRASE   & 94.8          & 90.0          & 92.3          & 83.7          & 61.9          & 71.1          \\\midrule
\textbf{FGWEA}    & \textbf{95.2} & \textbf{90.3} & \textbf{92.7} & \textbf{93.9} & \textbf{73.2} & \textbf{82.3} \\\bottomrule
\end{tabular}
}
% \vspace{-2mm}
\caption{Results on cross-source EA datasets.}\label{tab:exp3}
% \vspace{-5mm}
\end{table}


==> ACL23 Entity Alignment Camera Ready/tab_exp4.tex <==
\begin{table*}[t!]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccr|cccr|rrrr|rrrr}\toprule
            & \multicolumn{4}{c|}{DBP15K$_\textnormal{ZH\_EN}$}                        & \multicolumn{4}{c|}{SRPRS$_\textnormal{EN\_FR}$}                        & \multicolumn{4}{c|}{D-W-15K-V2}                                           & \multicolumn{4}{c}{MED-BBK-9K}                     \\
Model       & Hit1           & Hit10          & MRR            & Time & Hit1           & Hit10          & MRR            & Time & P             & R             & $F_1$            & Time           & P             & R             & $F_1$            & Time                 \\\midrule
FGWEA   & \textbf{0.987} & \textbf{0.997} & \textbf{0.991} & 254  & \textbf{0.996} & \textbf{0.999} & \textbf{0.997} & 388  & 95.2          & \textbf{90.3} & \textbf{92.7} & 494                      & \textbf{93.9} & \textbf{73.2} & \textbf{82.3} & 151                  \\
- w/o GW     & 0.975          & 0.992          & 0.981          & 57   & 0.979          & 0.989          & 0.983          & 62   & 95.8          & 84.7          & 89.9          & 49                       & 92.4          & 58.5          & 71.7          & 19                   \\
- w/o $S_{rel}$  & 0.970          & 0.990          & 0.977          & 52   & 0.976          & 0.987          & 0.980          & 49   & \textbf{98.7} & 82.2          & 90.0          & 44                       & 92.6          & 57.8          & 71.1          & 18                   \\
- w/o $S_{stru}$ & 0.951          & 0.979          & 0.962          & 40   & 0.966          & 0.982          & 0.972          & 23   & 97.5          & 56.6          & 71.6          & 25                       & 89.4          & 45.2          & 60.1          & 10                   \\
\midrule
GW-only     & 0.011          & 0.026          & 0.017          & 555  & 0.004          & 0.023          & 0.011          & 504  & 0.3           & 0.1           & 0.1           & 227                      & 0.3           & 0.1           & 0.1           & 470                  \\
Emb-Match   & 0.763          & 0.861          & 0.799          & 1    & 0.915          & 0.959          & 0.931          & 1    & 57.3          & 57.3          & 57.3          & 1                        & 51.1          & 51.1          & 51.1          & 1            \\\bottomrule       
\end{tabular}
}
% \vspace{-2mm}
\caption{Ablation study of FGWEA. The wall-clock time is measured in seconds.}
% \vspace{-4mm}
\label{tab:exp4}
\end{table*}


